Correlations and dynamics of tunnel-coupled one-dimensional Bose gases

We present a series of experiments performed with two ultracold one-dimensional Bose gases (rubidium atoms) in a double well potential. Employing matter-wave interference, we can measure the spatially resolved phase difference between the two gases and consequently investigate spatial correlations. By investigating whether higher order correlation functions can be factorized into correlations of lower order, we can investigate the interaction properties of the system. For a non-interacting system, all correlation functions with orders greater than two factorize and one observes Gaussian fluctuations. Here, we present the measurement of non-factorizing fourth-order correlation functions, leading to an experimental characterization of the interactions between the collective excitations of the quantum many-body system. The degree of non-factorizibility, i.e., the degree of non-Gaussianity of the phase fluctuations, depends on the tuneable tunneling strength between the wells. Starting from such a non-Gaussian state, we are able to observe the dynamical evolution towards a state with factorizing correlation functions (Gaussian fluctuations). We start in a double well with tunneling and then abruptly decouple the two subsystems. Subsequently, we observe how the initially non-Gaussian phase fluctuations become Gaussian. Moreover, we discuss the dynamical emergence of phase coherence in a double well potential with tunneling. We experimentally investigate the evolution starting from two different initial states. In one case, we split a cloud of atoms into two and trigger global oscillations in their relative phase. The oscillations subsequently damp and phase coherence sets in. In the other case, two independent clouds are suddenly coupled by tunneling. Again, phase coherence emerges between the two subsystems.

==> outlook.tex <==
\chapter{Conclusion and outlook}
\label{chap:conclusion}


\subsection{Robustness}

\rt{
	\begin{itemize}
		\item reference to the Gaussification to argue that the observed curve is does not always appear
		\item emphasize that the fast cooled scans give different results, the results for a temperature much higher than what is measured from the density ripples, and much higher than what the imaging system can resolve
	\end{itemize}
}

\section{Outlook: 1PI correlations}

\rt{
	\begin{itemize}
		\item write about the general idea, that you want to get rid of the 'legs' of the diagrams
		\item write about that when only having access to the phases one can really only do this in classical fields approximation, but that J.Berges argued that one can also approx do it for the quantum case
		\item discuss what differences it makes that we are looking at phase-differences rather than phases itself, argue that one has to go to k-space and one has to assume that the 2p correlator is diagonal in order to be able to invert it
		\item present results of the cosine transformed higher connected parts
		\item present preliminary results?
	\end{itemize}
}

%\section{1PI correlations}

%\section{Publications connected to this thesis}
